TrUMAn: Trope Understanding in Movies and Animations

Understanding and comprehending video content is crucial for many real-world applications such as search and recommendation systems. While recent progress of deep learning has boosted performance on various tasks using visual cues, deep cognition to reason intentions, motivation, or causality remains challenging. Existing datasets that aim to examine video reasoning capability focus on visual signals such as actions, objects, relations, or could be answered utilizing text bias. Observing this, we propose a novel task, along with a new dataset: Trope Understanding in Movies and Animations (TrUMAn), with 2423 videos associated with 132 tropes, intending to evaluate and develop learning systems beyond visual signals. Tropes are frequently used storytelling devices for creative works. By coping with the trope understanding task and enabling the deep cognition skills of machines, data mining applications and algorithms could be taken to the next level. To tackle the challenging TrUMAn dataset, we present a Trope Understanding and Storytelling (TrUSt) with a new Conceptual Storyteller module, which guides the video encoder by performing video storytelling on a latent space. Experimental results demonstrate that state-of-the-art learning systems on existing tasks reach only 12.01% of accuracy with raw input signals. Also, even in the oracle case with human-annotated descriptions, BERT contextual embedding achieves at most 28% of accuracy. Our proposed TrUSt boosts the model performance and reaches 13.94% performance. We also provide detailed analysis to pave the way for future research. TrUMAn is publicly available at:https://www.cmlab.csie.ntu.edu.tw/project/trope

==> Figures/Backup.tex <==
%%Result.tex
\begin{table*}
  \caption{Experiment result}
  \label{exp.}
  \centering
  \begin{tabular}{c|ccc|c|cccccccc}
    \toprule
     & \multicolumn{3}{c|}{Modality} & \multicolumn{1}{c|}{Acc. in 5 folds} & \multicolumn{8}{c}{Category} \\
    \cmidrule(r){2-4}
    \cmidrule(r){6-13}
    Modal & Visual & Audio & Object & $Acc. \pm std$ & C. Trait & R. Inter & Scene/Obj & Story. U & Situ. U & Sent. & Audio & Def.\\
    \midrule
    Single modal & CNN & - & - & $9.33 \pm 1.06$ & 11.51 & 5.73 & 12.59 & 5.39 & 9.52 & 8.03 & 12.68 & 10.5 \\
    Single modal & C3D & - & - & $10.07 \pm 1.53$ & 11.23 & 8.33 & 14.81 & 6.47 & 10.59 & 8.03 & 13.74 & 8.84 \\
    Single modal & CNN+C3D & - & - & $10.57 \pm 1.89$ & 13.15 & 6.25 & 12.96 & 7.4 & 10.05 & 10.22 & 15.64 & 11.6 \\
    Single modal & - & ASR & - & $5.44 \pm 0.79$ & 9.86 & 5.73 & 6.3 & 3.24 & 3.96 & 8.76 & 8.67 & 2.21 \\
    Single modal & - & Sound & - & $4.13 \pm 0.89$ & 7.95 & 3.12 & 1.48 & 3.54 & 2.57 & 6.93 & 10.57 & 4.97 \\
    Single modal & - & - & FRCNN & $8.75 \pm 1.42$ & 11.23 & 5.73 & 12.22 & 5.7 & 8.77 & 8.76 & 12.47 & 10.5 \\
    \midrule
    Multi modal & CNN+C3D & ASR & - & $11.64 \pm 0.47$ & 14.52 & 8.85 & 15.56 & 8.63 & 11.02 & 12.04 & 15.43 & 10.5\\
    Multi modal & CNN+C3D & Sound & - & $9.21 \pm 1.09$ & 10.96 & 5.73 & 9.63 & 7.24 & 8.66 & 8.76 & 13.95 & 8.29\\
    Multi modal & CNN+C3D & - & FRCNN & $10.25 \pm 1.71$ & 13.97 & 9.38 & 9.26 & 6.78 & 10.59 & 9.85 & 18.18 & 9.39\\
    Multi modal & CNN+C3D & ASR & FRCNN & $12.39 \pm 2.06$ & 17.26 & 10.94 & 15.19 & 9.24 & 11.55 & 12.77 & 18.18 & 9.94\\
    Multi modal & CNN+C3D & Sound & FRCNN & $10.00 \pm 1.07$ & 13.15 & 8.85 & 10 & 5.86 & 9.95 & 8.76 & 16.07 & 13.26\\
    \midrule
    \multicolumn{4}{c|}{XDC \cite{xdc}} & \\
    \midrule
    \multicolumn{4}{c|}{Oracle (w/ written description)} & $27.84 \pm 2.14$ & 40.55 & 31.77 & 31.48 & 17.41 & 26.42 & 30.29 & 32.98 & 21.55\\
    \midrule
    \multicolumn{4}{c|}{Human} & \\
    \bottomrule
  \end{tabular}
\end{table*}

==> Figures/Human.tex <==
\begin{figure*} % I typically use ht
\includegraphics[width=\textwidth]{Figures/interface.png}
\caption{
{{\bfseries Our trope human evaluation interface.
}
}
}
\label{fig:inter}
\end{figure*}

==> Figures/Results.tex <==
\begin{table*}
  \centering
  \begin{tabular}{ccc|c|cccccccc}
    \toprule
     Method & \multicolumn{2}{c|}{Modality} & \multicolumn{1}{c|}{5-fold Acc} & \multicolumn{8}{c}{Category} \\
    \cmidrule(r){1-3}
    \cmidrule(r){4-12}
    & Visual & Audio  & $Acc. \pm std$ (\%) & C. Trait & R. Inter & Scene Id. & Story. U & Situ. U & Sent. & Audio & Mani.\\
    \midrule
    \multirow{7}{*}{Baseline} & CNN & - &  $9.33 \pm 1.06$ & 11.51 & 5.73 & 12.59 & 5.39 & 9.52 & 8.03 & 12.68 & 10.5 \\
     & C3D & - &  $10.07 \pm 1.53$ & 11.23 & 8.33 & 14.81 & 6.47 & 10.59 & 8.03 & 13.74 & 8.84 \\
     & CNN+C3D & - &  $10.57 \pm 1.89$ & 13.15 & 6.25 & 12.96 & 7.4 & 10.05 & 10.22 & 15.64 & 11.6 \\
     & - & ASR &  $5.44 \pm 0.79$ & 9.86 & 5.73 & 6.3 & 3.24 & 3.96 & 8.76 & 8.67 & 2.21 \\
     & - & Sound &  $4.13 \pm 0.89$ & 7.95 & 3.12 & 1.48 & 3.54 & 2.57 & 6.93 & 10.57 & 4.97 \\
     %- & - & FRCNN & $8.75 \pm 1.42$ & 11.23 & 5.73 & 12.22 & 5.7 & 8.77 & 8.76 & 12.47 & 10.5 \\
    %\midrule
    %\multicolumn{3}{c|}{VIOLIN multi-modal \cite{violin}} & $Acc. \pm std$ & C. Trait & R. Inter & Scene/Obj & Story. U & Situ. U & Sent. & Audio & Def.\\
     & CNN+C3D & ASR  & $11.64 \pm 0.47$ & 14.52 & 8.85 & 15.56 & 8.63 & 11.02 & 12.04 & 15.43 & 10.5\\
     & CNN+C3D & Sound  & $9.21 \pm 1.09$ & 10.96 & 5.73 & 9.63 & 7.24 & 8.66 & 8.76 & 13.95 & 8.29\\
    % CNN+C3D & - & FRCNN & $10.25 \pm 1.71$ & 13.97 & 9.38 & 9.26 & 6.78 & 10.59 & 9.85 & 18.18 & 9.39\\
     %CNN+C3D & ASR & FRCNN & $12.39 \pm 2.06$ & 17.26 & 10.94 & 15.19 & 9.24 & 11.55 & 12.77 & 18.18 & 9.94\\
     %CNN+C3D & Sound & FRCNN & $10.00 \pm 1.07$ & 13.15 & 8.85 & 10 & 5.86 & 9.95 & 8.76 & 16.07 & 13.26\\
    \midrule
    \multicolumn{3}{l|}{L-GCN \cite{L-GCN2020AAAI}} & $8.75 \pm 1.42$ & 11.23 & 5.73 & 12.22 & 5.7 & 8.77 & 8.76 & 12.47 & 10.5 \\
    \midrule
    \multicolumn{3}{l|}{L-GCN \cite{L-GCN2020AAAI} + Baseline} & $12.39 \pm 2.06$ & 17.26 & 10.94 & 15.19 & 9.24 & 11.55 & 12.77 & 18.18 & 9.94\\
    \midrule
    \multicolumn{3}{l|}{XDC \cite{xdc}} & $7.35 \pm 0.52$ & 10.96 & 3.12 & 6.67 & 5.86 & 5.88 & 7.30 & 15.22 & 6.63 \\
    \midrule
    \multicolumn{3}{l|}{Oracle (w/ written description)} & $27.84 \pm 2.14$ & 40.55 & 31.77 & 31.48 & 17.41 & 26.42 & 30.29 & 32.98 & 21.55\\
    \midrule
    %\multicolumn{3}{l|}{Human (Visual)} & 84.21 & \multicolumn{8}{c|}{-}\\
    %\multicolumn{3}{l|}{Human (Audio)} & 52.87 & \multicolumn{8}{c|}{-}\\
    %\multicolumn{3}{l|}{Human (Visual+Audio)} & 79.31 & \multicolumn{8}{c|}{-}\\
    %52.87 84.21 79.31
    \bottomrule
  \end{tabular}
  \caption{The experimental result with 5-fold cross validation. First block: The baseline model. The single-modal model has 10.57\% accuracy at best with CNN+C3D features. The multi-modal model reaches 11.64\% accuracy by leveraging multi-modal input signals. Second block: L-GCN \cite{L-GCN2020AAAI}, a state-of-the-art Video QA model, gets 8.75\% accuracy by utilizing detected object features. Third block: Combining L-GCN as a stream of the baseline model and fuse its output with the CNN+C3D visual feature and the ASR audio feature further boosts the performance to 12.39\% accuracy. Fourth block: XDC \cite{xdc}, a state-of-the-art self supervised action recognition model with audio-video cluster pretraining while performing significantly better on audio category, only has 7.35\% accuracy overall. Last block: Oracle case accessing human-written descriptions could achieve 27.84\% accuracy, which is remarkably better than all compared methods. (See Section \ref{section:experiment:results})
  %XDC, oracle, human
  }
  \label{tab:exp}
\end{table*}

==> Figures/Results_pseudocap.tex <==
\begin{table*}
  \centering
  \begin{tabular}{c|c|cccccccc}
    \toprule
    \multirow{2}{*} {Method} & \multicolumn{1}{c|}{5-fold Acc} & \multicolumn{8}{c}{Category} \\
    \cmidrule(r){2-10}
     & $Acc. \pm std$ (\%) & C. Trait & R. Inter & Scene Id. & Story. U & Situ. U & Sent. & Audio & Mani.\\
    \midrule
    \multicolumn{1}{l|}{Baseline (S3D + ASR)}  & $12.01 \pm 0.90$ & 13.97 & 10.42 & 14.44 & 8.78 & 11.12 & 14.23 & 20.93 & 11.60\\
    % \midrule
    \multicolumn{1}{l|}{\ourmodelabbr (S3D+ASR)} & $12.88 \pm 0.72$ & 17.26 & 19.79 & 9.63 & 10.63 & 10.91 & 17.52 & 26.00 & 7.18\\
    \midrule
    \midrule
    \multicolumn{1}{l|}{Baseline (S3D + ASR + LGCN)} & $12.50 \pm 0.52$ & 18.90 & 16.15 & 12.59 & 10.48 & 11.44 & 12.04 & 20.08 & 11.60\\
    % \midrule
    \multicolumn{1}{l|}{\ourmodelabbr (S3D+ASR+LGCN)} & $13.94 \pm 1.78$ & 19.73 & 16.67 & 15.93 & 10.32 & 13.69 & 18.98 & 20.72 & 13.26 \\
    \bottomrule
  \end{tabular}
  \caption{The ablation study for \ourmodelabbr. First block shows our \ourmodelabbr compares to  . (See Section \ref{section:experiment:results})
  %XDC, oracle, human
  }
  \label{tab:exp}
\end{table*}


% 13.5+-1.29
% 18.90 16.15 12.59 10.48 11.44 12.04 20.08 11.60
% 22.19 17.19 14.81 10.02 11.76 16.06 22.41  9.39
% 19.73 16.67 15.93 10.32 13.69 18.98 20.72 13.26

==> Figures/figcate.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/figcate_fig.pdf}
    \caption{{\bfseries The number of tropes in different category.} (See Section \ref{section:dataset:analysis})}
    \label{fig:figcate}
\end{figure}

==> Figures/interface.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/interface_fig.pdf}
    \caption{{\bfseries Our trope human evaluation interface.} Annotators are instructed to select confidence score and answer depends on the assigned modalities. (See Section \ref{section:experiment:methods})}
    \label{fig:inter}
\end{figure}

==> Figures/statistic.tex <==
\begin{table}[ht]
    \centering
    \noindent
        \begin{tabular}{c|ccccc}
        \toprule
        %&& Tropes & Words & Sentences & Roles & Mentions \\
        Data Split & Median & Average & Min & Max & \(\sigma\) \\
        \midrule
        1 & 53.33 & 62.32 & 4.00 & 233.67 & 43.29 \\
        2 & 54.33 & 65.54 & 3.67 & 151.00 & 43.94  \\
        3 & 53.00 & 60.70 & 3.67 & 187.33 & 41.22   \\
        4 & 51.67 & 61.58 & 4.33 & 237.66 & 42.89   \\
        5 & 49.00 & 60.01 & 3.67 & 154.67 & 41.64   \\
        \midrule
        All & 52.00 & 61.90 & 2.33 & 237.67 & 42.71   \\
        \bottomrule
        \end{tabular}
    \caption{{\bfseries\ourdatasetabbr{} dataset video statistics.} It shows the statistic of video length (in second) in each data split. The average video length is long and standard deviation is quite large.  (\(\sigma\) denotes standard deviation.) (See Section \ref{section:dataset:analysis})}
    \label{tab:statistic}
\end{table}

==> Figures/statisticcate.tex <==
\begin{table}[ht]
    \centering
    \noindent
        \begin{tabular}{l|ccccccccc}
        \toprule
        %&& Tropes & Words & Sentences & Roles & Mentions \\
        Cate. & C.T. & R.I. & S./O. & S.U. & S.L. & Sent. & Aud. & Man. & All \\
        \midrule
        Mid & 533 & 622 & 400 & 233 & 432 & 622 & 400 & 233 & 52\\
        Avg & 543 & 654 & 367 & 151 & 439 & 622 & 400 & 233 & 61 \\
        Min & 530 & 600 & 367 & 187 & 412 & 622 & 400 & 233 & 2  \\
        Max & 517 & 618 & 433 & 237 & 429 & 623 & 400 & 233 & 237  \\
        \(\sigma\) & 490 & 601 & 367 & 156 & 416 & 632 & 400 & 3.7 & 42  \\
        \bottomrule
        \end{tabular}
    \caption{{\bfseries\ourdatasetabbr{} dataset video statistics.} It shows the statistic of video length (in second) in each data split. The average video length is long and standard deviation is quite large.  (\(\sigma\) denotes standard deviation.) (See Section \ref{section:dataset:analysis})}
    \label{tab:statisticcate}
\end{table}
